Structural Diagnosability Analysis of Switched and Modular Battery Packs

Safety, reliability, and durability are targets of all engineering systems, including Li-ion batteries in electric vehicles. This paper focuses on sensor setup exploration for a battery-integrated modular multilevel converter (BI-MMC) that can be part of a solution to sustainable electrification of vehicles. BI-MMC contains switches to convert DC to AC to drive an electric machine. The various configurations of switches result in different operation modes, which in turn, pose great challenges for diagnostics. The study explores diverse sensor arrangements and system configurations for detecting and isolating faults in modular battery packs. Configurations involving a minimum of two modules integrated into the pack are essential to successfully isolate all faults. The findings indicate that the default sensor setup is insufficient for achieving complete fault isolability. Additionally, the investigation also demonstrates that current sensors in the submodules do not contribute significantly to fault isolability. Further, the results on switch positions show that the system configuration has a significant impact on fault isolability. A combination of appropriate sensor data and system configuration is important in achieving optimal diagnosability, which is a paramount objective in ensuring system safety.

==> Problem_formulation.tex <==
\section{Problem formulation}







	In Section III, a BI-MMC which is the focus of this paper will be introduced. The BI-MMC is modeled by Differential Algebraic Equations (DAE); and it can be in four feasible modes. Its default sensor setup is chosen for control perspectives. However, addintional sensor setup might be needed from diagnosis perspectives. \\
	Besides, each SM has four possible modes. So, a battery pack with $n$ SMs can have $4^n$ configurations in the fault-free case in total. Analysis and synthesis of all configurations are inefficient and/or infeasible. Therefore, analysis and synthesis of the diagnosis system should be limited to those configurations which are applicable and useful.
	     
	
	

